IML-ViT: Benchmarking Image Manipulation Localization by Vision Transformer

Advanced image tampering techniques are increasingly challenging the trustworthiness of multimedia, leading to the development of Image Manipulation Localization (IML). But what makes a good IML model? The answer lies in the way to capture artifacts. Exploiting artifacts requires the model to extract non-semantic discrepancies between manipulated and authentic regions, necessitating explicit comparisons between the two areas. With the self-attention mechanism, naturally, the Transformer should be a better candidate to capture artifacts. However, due to limited datasets, there is currently no pure ViT-based approach for IML to serve as a benchmark, and CNNs dominate the entire task. Nevertheless, CNNs suffer from weak long-range and non-semantic modeling. To bridge this gap, based on the fact that artifacts are sensitive to image resolution, amplified under multi-scale features, and massive at the manipulation border, we formulate the answer to the former question as building a ViT with high-resolution capacity, multi-scale feature extraction capability, and manipulation edge supervision that could converge with a small amount of data. We term this simple but effective ViT paradigm IML-ViT, which has significant potential to become a new benchmark for IML. Extensive experiments on three different mainstream protocols verified our model outperforms the state-of-the-art manipulation localization methods. Code and models are available at https://github.com/SunnyHaze/IML-ViT.

==> tables/protocol1_auc.tex <==
\begin{table}[h]
\centering

\resizebox*{0.5\columnwidth}{!}{ 
\begin{tabular}{@{}lll@{}}
\toprule[2pt]
\textbf{Method}      & \textbf{Pre-train}           & \textbf{$F_1$(\%)} \\ \midrule
RGB-N, CVPR18~\cite{RGBN_2018}        & ImageNet                             & 40.8                   \\
SPAN, ECCV20~\cite{SPAN_2020}        & Private synthesized dataset          & 38.2                   \\
Objectformer, CVPR22~\cite{objectformer_2022} & Private synthesized dataset          & 57.9                   \\
\textit{IML-ViT(Ours)}        & MAE on ImageNet-1k          & \textbf{72.0}                   \\ \bottomrule[2pt]
\end{tabular}
}
\caption{\textbf{Performance comparison with Closed-source methods} All the methods above are fine-tuning with CASIAv2 and are tested with the CASIAv1 dataset.  }
\label{tab:close}
\end{table}
